Optimizing Large-Scale Fleet Management on a Road Network using Multi-Agent Deep Reinforcement Learning with Graph Neural Network

We propose a novel approach to optimize fleet management by combining multi-agent reinforcement learning with graph neural network. To provide ride-hailing service, one needs to optimize dynamic resources and demands over spatial domain. While the spatial structure was previously approximated with a regular grid, our approach represents the road network with a graph, which better reflects the underlying geometric structure. Dynamic resource allocation is formulated as multi-agent reinforcement learning, whose action-value function (Q function) is approximated with graph neural networks. We use stochastic policy update rule over the graph with deep Q-networks (DQN), and achieve superior results over the greedy policy update. We design a realistic simulator that emulates the empirical taxi call data, and confirm the effectiveness of the proposed model under various conditions.

==> 02_related_works_old.tex <==
\section{Related Works}
\label{sec:related_works}

\subsection{Smart transportation system}
 As machine learning has been rapidly developed in recent few years, there are a lot of studies that tried to apply machine learning in traffic problems. Because the nature of many traffic problems is about many vehicles, multi-agent RL is usually used to handle it. With multi-agent RL, \cite{bakker2010traffic} dealt with traffic light control, while \cite{maciejewski2013influence, seow2009collaborative} tried to solve taxi dispatch problem. \cite{godfrey2002adaptive} used adaptive dynamic programming for dynamic fleet management. Piecewise linear function approximation was used to calculate future return. 
 \cite{wang2019large} used MARL to traffic signal control.
 %\cite{xu2018large} studied efficient dispatch algorithm in on-demand ride hailing service. They regarded order dispatch as a sequential decision making problem and used centralized algorithm to make decision. They calculated state value from historical data and used combinatorial optimizing algorithm in dispatch planning.
 As mentioned before, our work is largely inspired by \cite{lin2018efficient}. \cite{lin2018efficient} proposed contextual multi-agent RL which considers two type of contexts(geographic and collaborative) to prevent invalid actions. They applied their method to two widely used deep RL algorithms, DQN and actor-critic algorithm, and called it cDQN and cA2C. They designed a grid-shaped city simulator and showed that their proposed models were best. However this work have two problems. First one is that when they applied their model to DQN, they just sent all the agents to the maximum $Q$ value direction. Another problem is that they used several unrealistic assumptions, such as grid-shaped space and too sparse time step. In this paper we have improved above shortcomings by introducing a stochastic policy model on a road network graph.
 \cite{xu2018large} studied efficient dispatch algorithm in on-demand ride hailing service. They regarded order dispatch as a sequential decision making problem and used centralized algorithm to make decision. They calculated state value from historical data and used combinatorial optimizing algorithm in dispatch planning.
 \cite{li2019efficient} proposed cooperative multi-agent RL algorithm which adopted mean field approximation to model agents' interaction.
 \cite{ke2019optimizing} adopted delayed order matching and established two-stage framework that utilizes both multi agent RL and combinatorial method.
 
 
 \subsection{Multi-agent reinforcement learning}
 In multi-agent reinforcement learning, many agents interact with an environment and get reward. \cite{tan1993multi} is one of the first paper that dealt with multi-agent scheme. It proposed cooperative Q-learning that agents share policy and experience, which showed better performance on joint task compared to independent Q-learning. \cite{foerster2018counterfactual} used counterfactual multi-agent policy gradient model which comprised of centralized critic and decentralized actor. \cite{lowe2017multi} also used similar approach to \cite{foerster2018counterfactual}, adding extra information in training phase. However these works are limited to small number of agents because of communication cost. In order to treat more agents, it is a common approach to assume homogeneous agent in order to reduce the complexity. \cite{zheng2018magent} made a multi-agent simulation platform called MAgent, and evaluated several different DRL algorithms. While, \cite{yang2018mean} proposed mean-field Q-learning(MF-Q) and mean-field actor-critic(MF-AC) and had experimentally shown that these models converge to Nash equilibrium.
 Several works adopted graph neural network on MARL to  model environment of multi agents \cite{jiang2018graph, malysheva2019magnet}. 

\subsection{Stochastic policy RL}
In some cases, including a large-scale fleet management task, greedy policy is not an optimal solution. Policy based RL such as actor-critic or A3C~\cite{mnih2016asynchronous}, there is an additional network that approximates policy, so it is not that big problem. In value based RL, the most popular approach that introduced stochasticity is soft $Q$-learning \cite{haarnoja2017reinforcement}. Soft Q-learning added entropy term and expresses optimal policy via Boltzmann distribution. According to 
\cite{schulman2017equivalence}, we can get optimal policy by updates similar to standard Q-learning.

In this paper, we did not tried policy based RL because it was challenging to apply it to a graph neural network. Instead, we approximated policy using function of Q values and experimentally showed that still this approximation is effective.

\subsection{Graph neural network}
In recent years, we have witnessed the success of convolutional neural network in various tasks such as image segmentation, classification and generation. Inspired by the success of CNN, some researchers have conducted a study to apply similar method on graph-structed data. \cite{kipf2016semi} presented a Graph Convolutional Network(GCN), the basic graph neural network. It aggregates neighbors' representation and passes it through non-linear function. Graph Attention Network(GAT)\cite{velivckovic2017graph} introduced attention mechanism to GCN and increased model expression power. There are a lot of other recent works such as Relational-GCN\cite{schlichtkrull2017modeling}
, LGNN\cite{chen2017supervised} and SSE\cite{dai2018learning}, but we used the two most basic graph neural network, GCN and GAT in this paper.

==> table_algos/04_algo_1.tex <==
\begin{algorithm}
\caption{Modified DQN with stochastic policy update}\label{euclid}
\begin{algorithmic}[1]
\State Initialize $Q$ with $\theta$
\State Initialize $Q'$ with ${\theta}'=\theta$
\For{$m = 1$ to maxiter}
    \State Reset environment and observe initial state $s_0$.
    \For{$t = 0$ to $T$}
        \State Calc $Q^\pi(s_t, l_j; \theta)$ from $s_t$
        \State Calc ${\pi}(l_j \rightarrow l_k|s_t;\theta)$ from $Q^\pi(s_t, l_j; \theta)$
        %using Eq.(\ref{eq:our_policy_update})
        \State Sample next action $a_t$ from $\pi$
        \State Apply action $a_t$ and observe $R_t, s_{t+1}$
        \State Calc $Q^{\pi'}(s_{t+1}, l_j; {\theta}')$ from $s_{t+1}$
        \State Calc ${\pi}'(l_j \rightarrow l_k |s_{t+1};\theta')$ from $Q^{\pi'}(s_{t+1}, l_j; {\theta}')$
        %using Eq.(\ref{eq:our_policy_update})
        %\State \text{For each road $l_j$, compute $\mathbb{E}[Q'(l_j \rightarrow l_k, t+1)]$  from $Q'(l_j, t+1; {\theta}')$ and ${\pi}'(l_j \rightarrow l_k, t+1)$}
        % \For{\text{each road $l_j$}}
        %     \State$\text{Compute }{\pi}'(l_j, t+1)\text{ from }Q'(l_j, t+1; \theta)$
        %     \State$\text{Compute expected return }T(l_j)\text{ by (2)}$
        % \EndFor
        \For{each idle driver $i=1$ to $N_t$}
            \State Set
            $y_t^i= 
            \begin{dcases}
                R_t^i \; (=1),  & \hspace{-0.5em}\text{if get call}\\
                {\gamma} \hat{Q}^{\pi'}(s_{t+1}, l_{t+1}^i, i;{\theta}'),  &\hspace{-0.5em} \text{otherwise}
            \end{dcases}$
        \EndFor
        %\State\text{Calculate $Q_{target}$ at each road}
        \State Update $\theta$ by a gradient descent on loss function
        
        \hspace{1em}$\sum_{i=1}^{N_t}{[ {y_t^i} - Q^\pi(s_t, l^i_{t+1};\theta)]^2}$
        %$\sum_{i=1}^{N_t}{\left[ {y_t^i} - Q^\pi_{a^i_t}(s_t;\theta)\right]^2}$
        %loss by Eq (\ref{equ:mse_dqn}).}
        \State Update ${\theta}' \leftarrow \theta$ if needed
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

==> table_algos/06_exp_table_3.tex <==
\begin{table}[]
\caption{Performance comparison of \textbf{Exp} vs \textbf{Entropy} and GCN vs GAT.
}
\label{table:ExpEntropy}
\begin{center}
\begin{tabularx}{\textwidth}{ccccccc}
\hline
     & \multicolumn{2}{c}{100\% driver} & \multicolumn{2}{c}{50\% driver} & \multicolumn{2}{c}{20\% driver} \\
$\beta$ & Exp             & Entropy        & Exp            & Entropy        & Exp            & Entropy        \\
\hline\hline
50   & 0.776         & 0.780          & 0.575         & 0.580         & 0.297         & 0.298         \\
20   & 0.791         & 0.783          & 0.592         & 0.588         & 0.305         & 0.304         \\
10   & 0.782         & 0.759          & 0.583         & 0.563         & 0.300         & 0.293         \\
5    & 0.775         & 0.657          & 0.578         & 0.465         & 0.300         & 0.256    \\
\hline
\end{tabularx}
\\
\vspace{1em}
\\
\begin{tabular}{ccccccc}
\hline
        & \multicolumn{2}{c}{100\% driver} & \multicolumn{2}{c}{50\% driver} & \multicolumn{2}{c}{20\% driver} \\

$\beta$ & \hspace{0.35em}GCN\hspace{0.35em}             & \hspace{0.35em}GAT\hspace{0.35em}            & \hspace{0.35em}GCN\hspace{0.35em}            & \hspace{0.35em}GAT\hspace{0.35em}            & \hspace{0.35em}GCN\hspace{0.35em}            & \hspace{0.35em}GAT\hspace{0.35em}            \\
\hline
\hline
50      & 0.771           & 0.776          & 0.537          & 0.575          & 0.262          & 0.297          \\
20      & 0.778           & 0.791          & 0.546          & 0.592          & 0.267          & 0.305          \\
10      & 0.775           & 0.782          & 0.545          & 0.583          & 0.267          & 0.300          \\
5       & 0.773           & 0.775          & 0.546          & 0.578          & 0.268          & 0.300    \\
\hline
\end{tabular}
\end{center}
\end{table}
